Probabilistic programming interfaces for random graphs: Markov categories, graphons, and nominal sets

We study semantic models of probabilistic programming languages over graphs, and establish a connection to graphons from graph theory and combinatorics. We show that every well-behaved equational theory for our graph probabilistic programming language corresponds to a graphon, and conversely, every graphon arises in this way. We provide three constructions for showing that every graphon arises from an equational theory. The first is an abstract construction, using Markov categories and monoidal indeterminates. The second and third are more concrete. The second is in terms of traditional measure theoretic probability, which covers 'black-and-white' graphons. The third is in terms of probability monads on the nominal sets of Gabbay and Pitts. Specifically, we use a variation of nominal sets induced by the theory of graphs, which covers Erd\H{o}s-R\'enyi graphons. In this way, we build new models of graph probabilistic programming from graphons.

==> distribution_monad_semantics.tex <==
\paragraph*{Denotational semantics} We interpret types in this language as finite sets.
% Every set $X \in \Set$ is seen as a measurable space equipped with the discrete $\sigma$-algebra~$2^{X}$.
\begin{equation}
  \semD 1=\{\star\}
  \quad
  \semD {A\ast B}=\semD A\times \semD B
  \quad
  \semD {\tbool}=\{0,1\}\text.\label{eqn:finset}
\end{equation}

\begin{definition}[e.g.~\cite{jacobs-coalgebra}]\label{def:distribution-monad} The distribution monad $\DistM$ on $\Set$ is defined as follows:
\begin{itemize}
 \item On objects: each set $X$ is mapped to the set of all finitely-supported discrete probability measures $X$, that is, all functions $p : X \to \RR$ that are non-zero for only finitely many elements and satisfy $\sum_{x \in X} p(x) = 1$.
% \item On morphisms: $\DistM f：\DistM X \to \DistM Y$ is the pushforward: 
% \[
% \DistM f(p)(y) = \textstyle\sum_{x \in f^{-1}(y)} p(x)
% \] 
% for all $p \in \DistM X$, $f : X \to Y$, and $y \in Y$.
 \item The unit $\eta_X :  X\to \DistM (X)$ maps $x \in X$ to the indicator function 
 $\lambda y.\, [y=x]$, i.e.~the Dirac distribution~$\delta_x$.
 \item The bind function $(\bind)$ is defined as follows: 
 \[
         (f \bind g)(z)(y) = \textstyle\sum_{x \in X} f(z)(x) \cdot g(z,x)(y)
 \] 
%for $f\colon  Z \to \DistM(X)$, $g \colon Z {\times} X \to \DistM(Y)$, $z \in Z$, 
%${y \in Y}$.
% for all $f : Z \to \DistM(X)$, $g : Z \times X \to \DistM(Y)$, $z \in Z$
 %and $y \in Y$.
% \item The multiplication $\mu_X : \DistM^2X \to \DistM X$ is given by: 
% \[
% \mu_A(P)(x) = \sum_{p \in \DistM X} P(p) \cdot p(x)
% \] 
% for all $P \in \DistM^2(A)$ and $x \in X$.
 \end{itemize}
\end{definition}
By the standard construction for strong monads, each morphism $f : X \to Y$ 
gets mapped to $\DistM f：\DistM X \to \DistM Y$ that is the pushforward in this case: 
$\DistM f(p)(y) = \textstyle\sum_{x \in f^{-1}(y)} p(x)$.
%for all $p \in \DistM X$ and $y \in Y$.

% \paragraph*{Kleisli composition} A map $f：X \to \DistM Y$ is a probability kernel if for every $x \in X$, $f(x)(-) = f(x, -)$ is a probability distribution over $Y$. For two maps $f：X \to \DistM Y$ and $g： Y \to \DistM Z$, the composite is given by marginalizing over $\DistM Y$ (Chapman-Kolmogorov):
% \[
%   (g \comp f)(x)(z) = \sum_{y \in Y} f(x, y)\cdot g(y, z)
% \]

The semantics of the Bernoulli probabilistic language is in the Kleisli category of $\DistM$, where computations $\Gamma \vdash t: A$ are interpreted as maps $\semD{t} : \semD{\Gamma} \to \DistM\semD{A}$~\cite{moggi:computation_and_monads}. It follows the semantics described in Section~\ref{sec:monad}.

% \begin{proposition} $\Set$ is symmetric monoidal category with monoidal product given by cartesian product $X \tensor Y := X \times Y$. Then, the distribution monad $\DistM$ is left- and right-strong. Left-strength $l: X \times \DistM Y \to \DistM(X \times Y)$ sends a pair $(x, p)$ to a distribution $l(x, y) = l(x)(y)$. This gives a map $\productmeas: \DistM X \times \DistM Y \to \DistM(X \times Y)$, which, for a pair of marginal distributions over $X$ and $Y$, gives their product distribution.
% \end{proposition}

% \begin{proposition} There is also a map in the other direction $\marginal: \DistM(X \times Y) \to \DistM X \times \DistM Y$, which, for a distribution $p(-, -)$ over $X \times Y$ gives the pair of marginal distributions over $X$ and $Y$:
% \[
% \marginal(p) = \langle x \mapsto \sum_{y \in Y} p(-, y) , y \mapsto \sum_{x \in Y} p(x, -) \rangle
% \]
% \end{proposition}
% \todo[inline]{What are the properties of the marginal map?}

% \subsection{Semantics of the Bernoulli language}
% Semantics of the Bernoulli probabilistic programming language $\semD{-}$ is given in the Kleisli category for $\DistM$.
% \begin{itemize}

% \item $\semD{-}$ on types gives objects in $\Set$
%     \begin{align*}
%       \semD{\tbool} &= 1 + 1 \\
%       \semD{()} &= 1 \\
%       \semD{A * B} &= \semD{A}\times\semD{B}
%     \end{align*}

% \item $\semD{-}$ on contexts gives objects in $\Set$
%     \begin{align*}
%       \semD{-} &= 1 \\
%       \semD{\Gamma, (x: A)} &= \semD{\Gamma} \times \semD{A}
%     \end{align*}

% \item $\semD{\Gamma \vdash t: A}$ gives a Kleisli map $\semD{t} \in Hom(\semD{\Gamma}, \DistM\semD{A})$
%     \begin{align*}
%       \semD{\Gamma, (x_n: A_n), \Gamma' \vdash x_n: A_n} =& \eta_{A_n} \comp \pi_n \\
%       \semD{\Gamma \vdash \ttrue: \tbool} =& \eta_{\tbool} \comp \iota_1 \comp 1 \\
%       \semD{\Gamma \vdash \tfalse: \tbool} =& \eta_{\tbool} \comp \iota_2 \comp 1 \\
%       \semD{\Gamma \vdash (t_1, t_2): (A_1 * A_2)} =& s \comp \langle \semD{\Gamma \vdash t_1: A_1}, \semD{\Gamma \vdash t_2: A_2}\rangle \\
%       \semD{\Gamma \vdash \pi_1 t: A_1} =& \pi_1 \comp \marginal \comp \semD{\Gamma \vdash t: (A_1 \times A_2)} \\
%       \semD{\Gamma \vdash \pi_2 t: A_2} =& \pi_2 \comp \marginal \comp \semD{\Gamma \vdash t: (A_1 \times A_2)} \\
%       \semD{\Gamma \vdash \letin x t u: B} =& \semD{\Gamma, (x: A) \vdash u: B} \\
%       & \comp (id_\Gamma, \semD{\Gamma \vdash t : A}) \\
%       \semD{\Gamma \vdash \tbernoulli_r(): \tbool} =& (r\delta_{\iota_1} + (1-r)\delta_{\iota_2}) \comp 1 \\
%       \semD{\Gamma \vdash \ite u {t_1} {t_2} A} =& (\semD{\Gamma \vdash t_1: A} + \semD{\Gamma \vdash t_2: A}) \\
%       & \comp (\semD{\Gamma \vdash u: \tbool} \times id) \comp \Delta_{\semD{\Gamma}}
%       \end{align*}
% \end{itemize}
% In case of deterministic terms, we simply lift the semantics in finite sets by $\eta$. If the term does not depend on the context, we pre-compose with $1: \Gamma \to 1$. In the let case, given a map $\semD{ u }: \semD{\Gamma} \to \DistM(1 + 1)$ and two maps $\semD{t_1}, \semD{t_2} : \semD{\Gamma} \to \DistM\semD{A}$ we have to give a map $\semD{\Gamma} \to \DistM\semD{A}$; it is constructed as the composition:
% \begin{align*}
%   \semD{\Gamma}
%   \xrightarrow{\Delta_{\semD{\Gamma}}}
%   \semD{\Gamma} \times& \semD{\Gamma}
%   \xrightarrow{(\semD{u} \times id)}
%   2 \times \semD{\Gamma} \simeq \\
%   &\simeq  \semD{\Gamma} + \semD{\Gamma} \xrightarrow{\semD{t_1} + \semD{t_2}}
%   G\semD{A}
% \end{align*}
Since we interpret types in the language as finite sets, the Kleisli morphisms are just stochastic matrices, that is, matrices where each row sums to $1$. Therefore, terms $\Gamma\vdash t:A$ can be seen as matrices
$  \semD t\in \RR^{\semD{\Gamma }\times \semD A}$
%\begin{equation}
%\end{equation}
and the Kleisli composition is then just matrix multiplication.

